Adversarial Examples in Remote Sensing

This paper considers attacks against machine learning algorithms used in remote sensing applications, a domain that presents a suite of challenges that are not fully addressed by current research focused on natural image data such as ImageNet. In particular, we present a new study of adversarial examples in the context of satellite image classification problems. Using a recently curated data set and associated classifier, we provide a preliminary analysis of adversarial examples in settings where the targeted classifier is permitted multiple observations of the same location over time. While our experiments to date are purely digital, our problem setup explicitly incorporates a number of practical considerations that a real-world attacker would need to take into account when mounting a physical attack. We hope this work provides a useful starting point for future studies of potential vulnerabilities in this setting.

==> attack_model.tex <==
In this work we focus on targeted attacks; however, given the challenges posed by attacking entire sequences with a single patch we also track metrics related to overall classification rate (not just targeted attack success rate).

\subsubsection{Classification Loss}

\subsubsection{Segmentation Loss}

\subsubsection{Visual Subtlety}

Describe our "adversarial quilt" model - patch consisting of piecewise constant elements. (in ground plane space)

Describe conceptual difference by designing patch in physical coordinates.   Small but important distinction from prior work.

Describe in slightly more detail  the idea of \emph{expectation over transformation (EOT)}  \cite{athalye2017synthesizing} and how it can be used to build robust "patch-like" attacks.
Describe important sources of invariances in our setting (e.g. seasonal, cloud cover, azimuth, etc.) and how some others are less critical (e.g. range).

\[
\delta = \mathbb{E}_{t \sim T} \left[ d(t(x) - t(x'))\right],
\]
where $T$ is a distribution of transformation functions , for example random rotation, translation or additive noise.
In our setting, $T$ includes more the more complex transformations of slowly changing geographic dynamics (e.g. seasonal variation, foliage loss/gain, etc.).
This introduces a host of considerations from the remote sensing community.
Maybe add a reference to Wojtek's work here?
We also adopt the Lagrangian-relaxed form of the problem:
\[
x' = \underset{x}{\arg \min} \todo{working here}
\]


We have in mind a $n \times n$ meter square of material/paint that is piecwise constant on $1 \times 1$ meter regions (a  "quilt-like" construct).


